How much do charm sea quarks affect the charmonium spectrum?

The properties of charmonium states are or will be intensively studied by the B-factories Belle II and BESIII, the LHCb and PANDA experiments and at a future Super-c-tau Factory. Precise lattice calculations provide valuable input and several results have been obtained by simulating up, down and strange quarks in the sea. We investigate the impact of a charm quark in the sea on the charmonium spectrum, the renormalization group invariant charm-quark mass and the scalar charm-quark content of charmonium. The latter is obtained by the direct computation of the mass-derivatives of the charmonium masses. We do this investigation in a model, QCD with two degenerate charm quarks. The absence of light quarks allows us to reach very small lattice spacings down to 0.023 fm. By comparing to pure gauge theory we find that charm quarks in the sea affect the hyperfine splitting at a level below 2%. The most significant effects are 5% in the quark mass and 3% in the value of the charm quark content of the eta_c meson. Given that we simulate two charm quarks these estimates are upper bounds for the contribution of a single charm quark. We show that lattice spacings <0.06 fm are needed for safe continuum extrapolations of the charmonium spectrum with O(a) improved Wilson quarks. A useful relation for the projection to the desired parity of operators in two-point functions computed with twisted mass fermions is proven.

==> decoupling.tex <==
\begin{itemize}
 \item Theory of decoupling
 \item Applicability of PT
 \item Power corrections
 \item charm effects on charm observables
\end{itemize}

\subsection{Theory of decoupling}
If a quantum field theory (QFT) contains heavy degrees of freedom, but the energy scales of the 
physical processes one is interested in lie far below the masses of these heavy particles, it is often
advantegous to work with an effective theory instead of the fundamental one. The effective
theory is a QFT without the heavy degrees of freedom. Their effects are absorbed into the coupplings
and masses of the effective theory. The results obtained from the effective theory will coincide with those
of the fundamental one, up to corrections that are supressed by powers of the inverse heavy masses. This 
suppression is what makes particle physics feasible, because otherwise the knowledge of a yet undiscovered 
theory of 
everything would be required, before even the simplest low energy results could be obtained.

Various effective field theories are in use to approximate different corners of the standard model. Here 
we focus on the decoupling of heavy quarks from QCD. If the fundamental theory is QCD with Lagrangian
$\Lag_{\Nf}$, that describes $\Nf$ quark 
flavors, out of which one is heavy, with mass $M$, then the effective theory without the heavy quark
has the Lagrangian~\cite{}
\begin{equation}\label{eq:decLag}
   \Lag^{\rm eff} = \Lag_{\Nf-1} + \frac{1}{M} \Lag_1 + \frac{1}{M^2}\Lag_2 + \ldots \, .
\end{equation}
The parameters (masses and the coupling) of $\Lag_{\Nf-1}$ differ from those of the fundamental theory.
The additional Lagrangians $\Lag_i$, contain all possible local interactions of the light fields, that
are compatible with the symmetries of the fundamental theory. These interaction terms have mass dimension
$4+i$, and each comes with its own coupling. In practice \eq{eq:decLag} has to be truncated, to keep 
the number of couplings finite. This truncation is, what introduces the power corrections to 
the effective theory.

